PBEBench: A Multi-Step Programming by Examples Reasoning Benchmark inspired by Historical Linguistics

Although many benchmarks evaluate the reasoning abilities of Large Language Models (LLMs) within domains such as mathematics, coding, or data wrangling, few abstract away from domain specifics to examine reasoning as a capability in and of itself. We contribute a novel type of benchmark evaluating the inductive reasoning capabilities of LLMs that is inspired by the forward reconstruction task from historical linguistics but is formulated in an extremely simple, general way (in the form of Programming by Examples). The task involves generating a cascade of simple string rewrite programs to transform a given list of input strings into a list of desired output strings. We present a fully automated pipeline that programmatically generates problems of this type with controllable difficulty, enabling scalable evaluation of reasoning models while avoiding contamination. Using this approach, we construct two benchmarks: PBEBench-Lite, which efficiently stratifies models of varying capabilities, and PBEBench, which requires models to induce programs similar in complexity to those constructed by historical linguists. Our experiments reveal a substantial performance gap between models that leverage test-time compute or LCoT (long chain-of-thought) reasoning and those that do not. Moreover, although recent models show promise, the solve rate for both of them drops below 5% for hard instances of the PBEBench dataset (ground truth cascade lengths of 20 and 30, respectively), falling well short of realistic historical linguistics requirements even with computationally expensive, popular scaling techniques from the PBE and reasoning literature. Additionally, we also study the effectiveness of different scaling strategies and the impact of various hyperparameters on the difficulty of the generated data using gpt-oss-120b, the best-performing open-source model.

==> sections/000_abstract.tex <==
% \begin{abstract}
% Although many benchmarks evaluate the reasoning abilities of Large Language Models (LLMs), few abstract away from domain specifics to examine reasoning as a capability in and of itself.
% We contribute a novel type of benchmark evaluating the inductive reasoning capabilities of LLMs that is inspired by the forward reconstruction task from historical linguistics but is formulated in an extremely simple, general way (in the form of Programming by Examples or PBE).
% The task involves generating a cascade of simple string rewrite programs to transform a given list of input strings into a list of desired output strings.
% We present a fully automated pipeline that programmatically generates problems of this type with controllable difficulty and ordering constraints, enabling scalable evaluation of sequential inductive reasoning while avoiding contamination.
% Using this approach, we construct two benchmarks:
% \textit{PBEBench-Lite}, which efficiently stratifies models of varying capabilities, and \textit{PBEBench}, which requires models to induce programs more similar (in complexity) to those constructed by historical linguists. 
% Our experiments reveal a substantial performance gap between models that leverage test-time compute or LCoT (long chain-of-thought) reasoning and those that do not. 
% Moreover, although recent models such as gpt-oss-120b and GPT-5 show promise, the solve rate for both of them drops below 5\% for hard instances of the PBEBench dataset (ground truth cascade lengths of 20 and 30, respectively), falling well short of realistic historical linguistics requirements even with computationally expensive, popular scaling techniques from the PBE and reasoning literature.
% Finally, we also study the effectiveness of different scaling strategies, evaluate LLMs on real forward reconstruction data, and compare the predictive power of PBEBench against other relevant inductive reasoning benchmarks, and show that competitive reasoning models like GPT-5 and gpt-oss-120b fail to beat it.
% We plan to open-source our code and benchmark snapshots to enable reproducibility and future work.
% \end{abstract}
\begin{abstract}
While many benchmarks assess the reasoning abilities of Large Language Models (LLMs), few abstract away from domain specifics to study reasoning as a capability in itself. 
We introduce a new benchmark for inductive reasoning inspired by the forward reconstruction task in historical linguistics, formulated in a simple and general Programming by Example (PBE) setting. 
The task requires generating a cascade of simple string rewrite programs that transform input strings into target outputs. 
We present a fully automated pipeline that programmatically generates such problems with controllable difficulty and ordering constraints, enabling scalable, contamination-resistant evaluation of sequential inductive reasoning. 
Using this pipeline, we construct two benchmarks: \textit{PBEBench-Lite}, which efficiently stratifies models of varying capability, and \textit{PBEBench}, which requires inducing programs comparable in complexity to those produced by historical linguists. 
Experiments reveal a large gap between models that use test-time compute or long chain-of-thought reasoning and those that do not. 
Although recent models such as GPT-5 and gpt-oss-120b show promise, their solve rates fall below 5\% on hard \textit{PBEBench} instances, with ground-truth cascade lengths of 20 and 30, respectively, even when using computationally expensive scaling techniques from the PBE and reasoning literature.
We also evaluate models on real forward reconstruction data, and show that \textit{PBEBench} is more predictive of their performance than other inductive reasoning benchmarks. 
We plan to open-source our code and benchmark snapshots to support reproducibility and future work.
\end{abstract}


==> sections/001_intro.tex <==
\section{Introduction}

You are trying to refactor a large codebase, implementing changes like replacing all instances of \texttt{foo} with \texttt{bar}, \texttt{bar} with \texttt{baz}, and \texttt{baz} with \texttt{foo}. When you tell your senior colleague, a seasoned Unix hacker, what you are doing, he smiles and says that he can (after inspecting the originals and your examples of refactored code) write a \texttt{sed} (stream editor) script that will update the entire codebase. His task involves not only constructing the appropriate regular expression replacements, but also placing them in the correct sequence. For example, \texttt{s/bar/baz/} (replace all instances of \texttt{bar} with \texttt{baz}) has to be ordered before \texttt{s/foo/bar/} (otherwise, all instances that were originally \texttt{foo} would become \texttt{baz}). Likewise, there must be a substitution like \texttt{s/baz/TEMP/} that occurs at the beginning of the the ``cascade'' and one like \texttt{s/TEMP/foo} that occurs at the end (yielding a circular mapping). At a deep level, this problem is the same as one from historical linguistics: given a set of pairs consisting of a word in an ancestral language and a word in a modern language, define a sequence of local string transformations that convert the ancestral words to the modern words (a task called forward reconstruction). In both cases, one is given a collection of inputs $\vec{i}$ (input files or ancestral words) and a collection of outputs $\vec{o}$ to which the inputs should be mapped by a program $\vec{p}$ consisting of a sequence of incremental transformations. Both are clear instances of programming example, \cite{naik2025programming} (the inspiration for the current work) having made this explicit for forward reconstruction.

An important observation of \cite{naik2025programming} is that this class of tasks is challenging for LLMs. Because of this, and because it can be reduced to the barest formal machinery, it provides an ideal framework for comparing the ability of language models to construct (by induction) sequential plans. The principle contribution of the paper is a benchmark of this type. It has a number of desirable properties underrepresented in current benchmarks for reasoning: (1) Unlike most reasoning benchmarks (see \ref{sec:related-work}), it is not bound to a specific domain and does not benefit from non-trivial domain knowledge. (2) Its complexity and difficulty emerge from a very simple framework with provable logic. (3) This emergent complexity includes four fundamental challenges (to capture the relationships \cite{Kiparsky1968-KIPLUA,kiparsky1971historical} called feeding, bleeding, counter-feeding, and counter-bleeding) which can be manipulated and quantified. (4) The benchmark is immune to data contamination and resistant to saturation because new test instances can be generated, with controlled difficulty very efficiently. (5) It compares the ability of models to perform a class of practically and scientifically interesting tasks rather than focusing on comparisons between model and human abilities.

\phantomsection
\label{sec:introduction:research_questions}
Our study addresses the following questions:

\textbf{RQ1: Which models are good at inductive reasoning?} We benchmark 13 reasoning and 8 strong non-reasoning models on PBEBench-Lite (a lightweight version of the proposed benchmark) to determine whether long chain of thought (LCoT) reasoning is beneficial in this task. \\
\textbf{RQ2: What makes a PBE instance hard?} We use logistic regression and factorial analysis to determine how much factors like ground truth cascade length, types of relations between rewrites, etc., impact the solution difficulty of dataset problems, based on solution success across all models. We also create a snapshot similar to PBEBench-Lite but with 50 examples per PBE instance (PBEBench-Lite-MoreEg) to evaluate the impact of having more examples on solution success rate.\\
\textbf{RQ3: Could the strongest LLMs solve problems requiring long programs (like real-world forward reconstruction problems)?} We pick the strongest open and closed-source models from the PBEBench-Lite results and analyze them on PBEBench (the full benchmark). \\
\textbf{RQ4: What scaling strategies work best for solution search?} We investigate which of the two solution search scaling strategies discussed in Section~\ref{sec:program_induction:prompting} yields more ``bang for the buck'' by holding the sampling budget constant and varying the maximum sequence length and vice-versa.

==> sections/004_methodology.tex <==
\section{Methodology}
\label{sec:methodology}
Our approach consists of two components: (1) a problem proposer and (2) a problem solver. 
The proposer is a programmatic system that generates PBE instances of controllable difficulty, forming the core of our dynamic benchmarking framework. 
It scalably and reliably produces novel, contamination-free data of the desired complexity. 
The solver is any system under evaluation. 
In this work, we focus on state-of-the-art open and closed-source reasoning LLMs to examine the limits of their inductive reasoning capabilities and to assess whether LLM-based methods can be deployed for realistic historical linguistics sound law induction tasks.


\begin{figure*}[!tbh]
\centering
\includegraphics[width=0.8\columnwidth]{figures/PBEBench_Data_Instance_V2_Fixed.png}
\caption{Structure of the <$\vec{i},\vec{p},\vec{o}$> triples dataset. The relations between the programs in the sequence are shown by the BFCC DAG, and the simplified BF DAG replaces the counterfactual relations with a reversed simple link.}
\label{fig:data_instance}
\end{figure*}

% can change the section names accordingly
\subsection{Problem Proposer}
\label{sec:problem_proposer}
We construct our benchmark programmatically by sampling inputs from a distribution of strings $\mathcal{I}$ and a sequence of string rewrite programs from a distribution $\mathcal{P}$. 
Each string rewrite program acts like a find and replace function and substitutes all occurrences of substring $\alpha$ with a substring $\beta$ (details in Section~\ref{sec:program_sampling_and_output_generation}).
We apply the sampled \textit{cascade} of string rewrite programs $\vec{p}=\langle p_1,\dots,p_m\rangle \in \mathcal{P}$ to the sampled inputs $\vec{i}=\langle i_1,\dots,i_n\rangle \in \mathcal{I}$, producing outputs $\vec{o}=\{p_m(\dots p_1(i_1)), \dots, p_m(\dots p_1(i_n))\}$.
For convenience, we write this transformation as $\vec{o}=\vec{p}(\vec{i})$. 
Each instance in our dataset is defined by the triplet $\langle \vec{i}, \vec{p}, \vec{o} \rangle$, consisting of the inputs, the program cascade, and the corresponding outputs. 
Additionally, we record metadata such as the interactions between programs (e.g., \textsc{bleeding}, \textsc{feeding}, etc.). 

Our data generation algorithm is parameterized by: the number of examples $n$ ($|\vec{i}| = |\vec{o}| = n$); the input alphabet $\Sigma$ used to generate both the inputs and the string rewrite programs; the minimum and maximum input string lengths $l_{min}$ and $l_{max}$; the minimum and maximum cascade lengths $L_{min}$ and $L_{max}$ ($L_{min} \leq |\vec{p}| \leq L_{max}$); the minimum and maximum length of strings $s_{min}$ and $s_{max}$ ($s_{min}\leq|\alpha|,|\beta|\leq s_{max}$) used by the string rewrite programs and the desired dataset size $D$. 
We denote a benchmark snapshot generated with specific parameter values as $\mathcal{D}(n, \Sigma, L_{min}, L_{max}, l_{min}, l_{max}, s_{min}, s_{max}, D)$.

% Each example consists of five input strings, five corresponding output strings, a sequence of transformation rules, and a graph that encodes the interactions among these rules.
\subsubsection{Input Sampling}
\label{sec:methodology:input_sampling}
Our input sampling procedure is parameterized by $(n, \Sigma, l_{min}, l_{max})$ as defined in Section~\ref{sec:problem_proposer}. 
We build the input sequence $\vec{i} = \langle i_1, \dots, i_n \rangle$ by independently sampling each input $i_{k}$ for $1 \leq k \leq n$. 
For each $i_k$, we first sample its length from a uniform discrete distribution, $|i_k| \sim \mathrm{Unif}\{l_{min}, \dots, l_{max}\}$,
where $|i_k|$ denotes the length of the string $i_k$. 
We then generate the string itself by sampling $|i_k|$ characters independently with replacement from the alphabet $\Sigma$, i.e.,
$i_k \sim \mathrm{Unif}(\Sigma)^{|i_k|}$.
% Each input string is sampled independently, with a length uniformly drawn between 2 and 6 characters. Characters are sampled uniformly from a restricted alphabet (e.g., \texttt{abcdef ghijk xyz}). At this stage, the strings are unaltered; however, we ensure they are valid for subsequent transformation steps.
\subsubsection{Program Sampling and Output Generation}
\label{sec:program_sampling_and_output_generation}
Program sampling is parameterized by $(\Sigma, L_{min}, L_{max}, s_{min}, s_{max})$. 
We begin by programmatically selecting a cascade length $L$ such that $L_{min} \leq L \leq L_{max}$. 
Next, we construct a sequence of $L$ string rewrite programs $\vec{p} = \langle p_1, \dots, p_L \rangle$, where each program is of the form $p_k = \mathrm{replace}(\alpha_k, \beta_k)$. 
Here, $\mathrm{replace}$ has the same semantics as Python’s built-in \texttt{replace()} method for strings: the substring $\alpha_k$ is replaced by $\beta_k$, with the restriction that $\alpha_k$ is non-empty. 
To sample each program $p_k$, we generate $\alpha_k$ and $\beta_k$ independently, following a procedure analogous to input sampling:
\begin{enumerate}[itemsep=1pt, leftmargin=*, parsep=0pt, topsep=-2pt, partopsep=0pt]
    \item Sample the lengths $|\alpha_k|$ and $|\beta_k|$ from a discrete uniform distribution: $|\alpha_k|, |\beta_k| \sim \mathrm{Unif}\{s_{min}, \dots, s_{max}\}$

    \item Sample $\alpha_k$ uniformly from the set of substrings of length $|\alpha_k|$ in the intermediate input vector $\vec{i}_{k-1}=p_{k-1}(\dots p_1(\vec{i}))$ (where $\mathrm{Substr}_{s}(\vec{i}_{k-1})$ denotes the set of all substrings of length $s$ in $\vec{i}_{k-1}$): $ \alpha_k \sim \mathrm{Unif}(\mathrm{Substr}_{|\alpha_k|}(\vec{i}_{k-1}))$ (note that $\vec{i}_0 = \vec{i}$).

    \item Sample $\beta_k$ as a sequence of $|\beta_k|$ characters, each drawn independently from the uniform character distribution over the alphabet $\Sigma$ (same as in Section~\ref{sec:methodology:input_sampling}): $\beta_k \sim \mathrm{Unif}(\Sigma)^{|\beta_k|}$
\end{enumerate}
The outputs are then generated by executing the program cascade $\vec{p}$ over the inputs $\vec{i}$ as $\vec{o} = \vec{p}(\vec{i})$

% \subsubsection{Enforcing Complexity Constraints}
% We manipulate the complexity of the cascade of string rewrite programs $\vec{p}$, including interaction types such as \textsc{bleeding}, \textsc{feeding}, and others, using careful rejection sampling guided by the classifiers developed in Section~\ref{sec:theory}. We balance the generated data along two dimensions of complexity: (1) the length of the ground truth cascade (or sequence) of string rewrite programs $|\vec{p}|$, and (2) the set of relation types present in the data. The second dimension is encoded as a binary category string $c_p$. For example, $c_p=1101$ denotes a cascade containing at least one instance of feeding, bleeding, and counter-bleeding but none of counter-feeding. We balance instances across all 16 possible category strings, ranging from the simplest case $c_p=0000$ (no relations present, where the program sequence can be ordered arbitrarily) to the most complex case $c_p=1111$ (all relation types present, where program ordering is highly constrained).

% \label{sec:rejection_sampling}
% \textbf{Computing Instance Complexity:} We hypothesize that the difficulty of a given PBE problem ($\langle\vec{i}$,$\vec{p}$,$\vec{o}\rangle$) is controlled by two factors: 1) number of programs and 2) the types of relations between all pairs of programs in the program sequence $\vec{p}$.
% An important contribution of our work is provably correct and automatic classification of the types of relations between any given pair of string rewrite programs 
% (Section~\ref{sec:theory}). 

% For a given pair of programs $p_i$ and $p_j$ in the program sequence $\vec{p}$: \\
% \textbf{Feeding (F):} $p_i$ creates substrings that enable $p_j$ to apply.
% \\
% \textbf{Bleeding (B):} $p_i$ removes substrings that $p_j$ requires.
% \\
% \textbf{Counter-Feeding (CF):} $p_i$ could have fed $p_j$, but $p_j$ precedes $p_i$.
% \\
% \textbf{Counter-Bleeding (CB):} $p_i$ could have bled $p_j$, but $p_j$ precedes $p_i$.
% \\
% \textbf{No Relation:} $p_i$ and $p_j$ can be ordered in any way possible.

% We do not need to explicitly store or classify counter relations, since recording both $(p_i,p_j)$ (where $p_i$ is applied before $p_j$) and $(p_j,p_i)$ (where $p_j$ is applied before $p_i$) automatically captures them.
% We can also visualize the relationships between the rules using a Directed Acyclic Graph (DAG) as shown in Figure~\ref{fig:data_instance}.
% We show both the actual DAG with all relations and a simplified DAG that indirectly captures the counter relations using the strategy mentioned above.

% \textbf{Rejection Sampling to Control Complexity:} To control data complexity according to the factors outlined above, we apply rejection sampling as described in Section~\ref{sec:program_sampling_and_output_generation}. 
% Each example is associated with a category string $c_p$ (defined in Section~\ref{sec:program_sampling_and_output_generation}), represented as a 4-bit vector $c_p \in \{0,1\}^4$. 
% Using these categories, we generate data to roughly balance the distribution across the $2^4=16$ possible complexity categories. 
% Given a maximum cascade length $m$, we also attempt to balance the number of instances across ground truth cascade lengths ranging from $2$ to $m$. 

% However, these two constraints can conflict. For example, with a cascade length of $2$, it is unlikely to find program pairs that span all relation-type complexity categories, since such pairs rarely exhibit three or four relation types simultaneously. 
% This conflict often results in a high rejection rate, as many samples fail to satisfy both constraints, making it necessary to relax at least one of them. 
% To address this, we experimented with various strategies and ultimately adopted a patience parameter $\tau$ on the number of search steps. Once $\tau(=100000)$ is exceeded, we accept any instance that satisfies at least one of the constraints. 
% In initial experiments, we prioritized relation types, but subsequent analysis revealed that cascade length was more predictive of empirical difficulty. 
% Accordingly, in later experiments we relaxed the relation-type constraints while maintaining control over cascade length.
\subsubsection{Enforcing Complexity Constraints}
\label{sec:rejection_sampling}
We control the complexity of cascades of string rewrite programs $\vec{p}$ using rejection sampling guided by the classifiers developed in Section~\ref{sec:theory}. 
Complexity is balanced along two dimensions: 
(1) the cascade length $|\vec{p}|$, and 
(2) the set of relation types present between programs in $\vec{p}$. 
The second dimension is encoded as a binary category string $c_p \in \{0,1\}^4$.
Each digit corresponds to the binary presence or absence of feeding, bleeding, counter-feeding, and counter-bleeding relations.
% For example, $c_p=1101$ denotes a cascade containing at least one instance of feeding, bleeding, and counter-bleeding, but no counter-feeding. 
Instances are balanced across all 16 possible category strings, from $c_p=0000$ (no relations present, arbitrary ordering possible) to $c_p=1111$ (all relations present, ordering highly constrained).

\textbf{Computing Instance Complexity.} 
We hypothesize that the difficulty of a PBE problem $\langle \vec{i}, \vec{p}, \vec{o} \rangle$ is governed by (1) cascade length and (2) the types of relations between program pairs in $\vec{p}$ (relations formulated by phonologists and historical linguists; see \citet{Kiparsky1968-KIPLUA,kiparsky1971historical}). 
One key contribution is a provably correct and automatic classification of these relations (Appendix~\ref{sec:theory}). 
For any ordered pair of programs ($p_i$,$p_j$) in $\vec{p}$, the possible relations are:
\begin{itemize}[itemsep=1pt, leftmargin=*, parsep=0pt, topsep=-2pt, partopsep=0pt]
    \item \textbf{Feeding (F($p_i$, $p_j$):} $p_i$ creates substrings that enable $p_j$ to apply.
    \item \textbf{Bleeding (B($p_i$, $p_j$):} $p_i$ removes substrings required by $p_j$.
    \item \textbf{Counter-Feeding (CF($p_i$, $p_j$)):} $p_i$ could have fed $p_j$, but $p_j$ precedes $p_i$.
    \item \textbf{Counter-Bleeding (CB($p_i$, $p_j$)):} $p_i$ could have bled $p_j$, but $p_j$ precedes $p_i$.
    \item \textbf{No Relation:} $p_i$ and $p_j$ can be ordered arbitrarily.
\end{itemize}

Counter-relations need not be stored explicitly, since $CF(p_i, p_j)$ and $CB(p_i, p_j)$ are implied if $p_j$ precedes $p_i$ and $F(p_j, p_i)$ and $B(p_j, p_i)$, respectively. 
These relations can be visualized using a Directed Acyclic Graph (DAG), as illustrated in Figure~\ref{fig:data_instance}. 
We show both the full DAG with all relations and a simplified DAG that indirectly encodes counter-relations via this symmetry.

\textbf{Rejection Sampling to Control Complexity.} 
% To enforce balanced complexity, we apply rejection sampling as described in Section~\ref{sec:program_sampling_and_output_generation}. 
% Each instance is associated with a category string $c_p$, and data is generated to achieve an approximate balance across the $2^4=16$ possible relation-type categories. 
% Given minimun and maximum cascade lengths $L_{min}$ and $L_{max}$, we also aim to balance the distribution of cascades across them. These constraints may conflict.
% For example, with cascade length $L=2$, it is unlikely for randomly sampled program pairs to exhibit three or four relation types simultaneously, making certain category strings unattainable. Recent work on using LLMs for sound law induction \citep{naik2025programmingexamplesmeetshistorical} showed that fine-tuning on programs randomly sampled under a parametrized generation process lead to more improvements on real world forward reconstruction than retrieving programs from a database of known attested sound laws which the authors speculated was due to greater diversity of the randomly sampled programs. 
% Therefore, we also keep random sampling as an inherent part of our dataset generation process (instead of generating them deterministically or retrieving from a database of programs) to avoid possible data contamination and promote diversity.
% This results in high rejection rates, often requiring relaxation of constraints. 
% To address this, we introduce a patience parameter $\tau$ on the number of samples rejected. 
% Once $\tau (=100000)$ is exceeded, we accept any instance that satisfies at least one constraint (out of target category string $c_p$ and cascade length). 
% In early experiments, relation-type balancing was prioritized, but later analysis (Appendix~\ref{sec:appendix:logistic_regression}) showed that ground truth cascade length was a stronger predictor of difficulty. 
% Consequently, in subsequent experiments we relaxed relation-type constraints while maintaining strict control over cascade length.
To enforce balanced complexity, we use rejection sampling (Section~\ref{sec:program_sampling_and_output_generation}). 
Each instance is assigned a category string $c_p$, and data is generated to approximate balance across the $2^4=16$ relation-type categories. 
We also aim to balance cascade lengths between $L_{min}$ and $L_{max}$, though these constraints can conflict. 
For example, with $L=2$, randomly sampled program pairs rarely exhibit three or four relation types, making some category strings unattainable. 
Prior work on sound law induction \citep{naik2025programmingexamplesmeetshistorical} showed that fine-tuning on randomly sampled programs yielded greater improvements in real-world forward reconstruction than retrieving from attested sound laws, likely due to higher diversity. 
Following this insight, we retain random sampling (rather than deterministic generation or database retrieval) to promote diversity and avoid contamination. 
This leads to high rejection rates, often requiring constraint relaxation. 
We therefore introduce a patience parameter $\tau$, which is the number of sampling steps carried out with both constraints. 
Once $\tau (=100000)$ is exceeded, we accept any instance satisfying at least one constraint (either $c_p$ or cascade length). 
In early experiments, relation-type balance was prioritized, but later analysis (Appendix~\ref{sec:appendix:factorial_analysis}, \ref{sec:appendix:logistic_regression}) showed cascade length to be a stronger predictor of difficulty. 
Accordingly, in subsequent experiments, we relaxed relation-type constraints while maintaining strict control over cascade length.  
We also study the effect of using different values of $\tau$ on the balance of relation types and efficiency of the data generation process (Appendix~\ref{sec:appendix:efficiency}).
\subsection{Problem Solver}
\label{sec:program_induction:prompting}
\textbf{Prompting Strategy:} Once a benchmark snapshot $\mathcal{D}$ is generated, we evaluate each LLM $M$ by prompting it (see appendix~\ref{sec:appendix:method_details:prompt_template}) to produce a candidate program cascade $\hat{\vec{p}} = M(\vec{i}, \vec{o})$ mapping inputs $\vec{i}$ to outputs $\vec{o}$. 
The prompt enforces the following constraints: each program must be a Python \texttt{replace} function; both arguments $\alpha_k$ and $\beta_k$ must be strings with $|\alpha_k|, |\beta_k| \leq s_{max}$; $\alpha_k$ must be non-empty; the cascade may contain at most $L_{max}$ programs (matching the length of the longest ground-truth cascade); and the output must follow a strict Markdown format for reliable extraction. 
If a predicted program $\hat{p}_j$ has more than $L_{max}$ programs, we consider the first $L_{max}$ programs for evaluation. If the predicted program violates any other constraint, it is replaced by an identity program $p^I$, which leaves inputs unchanged. 
Given the predicted cascade $\hat{\vec{p}}$, we compute the predicted outputs as $\hat{\vec{o}} = \hat{\vec{p}}(\vec{i})$.
Since we evaluate all kinds of LLMs, including reasoning models that may first produce intermediate outputs and then iteratively refine or improve them by reflection, we account for this by evaluating both the first and last code block produced by each model.
% Details of program extraction from LLM responses are provided in appendix~\ref{sec:appendix:method_details:program_extraction}.

\textbf{Scaling Solution Search:} We explore two approaches to scaling the solution search, inspired by prior work on LLMs for PBE \citep{li2024is} and general reasoning \citep{muennighoff2025s1}: (1) sampling budget and (2) test-time thinking-budget scaling.  
The first approach gives the LLM multiple attempts to solve a problem by successively sampling solutions $K$ times and selecting any solution consistent with the input-output examples. If no correct solution is found in the $K$ samples, we pick the one with the highest edit similarity reward (defined in Section~\ref{sec:experiments:eval_metrics}).  
The second approach is inspired by \cite{muennighoff2025s1}. We constrain the thinking budget to $N$ tokens and scale it by increasing this limit. However, we observed that gpt-oss-120b does not strictly adhere to thinking budget constraint, even when employing strategies such as forcing it to emit chain-of-thought termination tokens (experimental details are available in Appendix \ref{sec:cot_truncation_experiment}), so we ultimately control the overall maximum sequence length.


% Local Variables:
% TeX-master: "../iclr2026_conference"
% TeX-engine: xetex
% mode: LaTeX
% End:


==> sections/006_future_work_and_limitations.tex <==
\section{Conclusion and Future Work}
% Firstly we observe that PBEBench-Lite alone is challenging for a lot of the evaluated models especially the non-reasoning models evaluate showing that inductive reasoning might necessitate some form long chain of though reasoning at test time. 
% Furthermore the experiments with the strongest open and closed source models on the more realistic PBEBench dataset reveal that while these models can successfully solve problems up to a certain complexity, their performance steadily drops off as the complexity (largely driven by ground truth cascade length) increases and despite comptuationally heavy scaling strategies like sampling budget and higher token budgets for longer chains of thought the performance eventually saturates and the model runs into reasoning barriers allowing us to assess the true limits of current state of the art reasoning models.
% However these results are promising and already show a lot of improvement over prior work like \citet{naik2024can, naik2025programming} which indicates a bright future for solving forward reconstruction problems with LLMs.
% Finally we note that the automated and scalable programmatic generation of data of controllable complexity with our pipeline opens up the possibility of generating more and more complex synthetic training data to improve the PBE and inductive reasoning capabilites of open weight reasoning models using a curriculum learning style strategy, which we plan to explore in future work.
% Firstly, we observe that PBEBench-Lite is already challenging for many evaluated models, especially non-reasoning ones, suggesting that inductive reasoning may require long chains of thought at test time. 
% Experiments with the strongest open and closed-source models on the more realistic PBEBench dataset further show that while these models solve problems up to a certain complexity, performance steadily declines as complexity (driven largely by ground-truth cascade length) increases. 
% Even with computationally intensive scaling strategies such as larger sampling and token budgets for longer chains of thought, performance eventually saturates, revealing reasoning barriers and exposing the true limits of current state-of-the-art models. 
% Nonetheless, these results are promising and already surpass prior work \citep{naik2024can, naik2025programming}, indicating a bright future for solving forward reconstruction problems with LLMs. 
% Finally, the automated, scalable generation of data with controllable complexity enabled by our pipeline opens the door to creating increasingly complex synthetic training data, which could enhance the PBE and inductive reasoning abilities of open-weight models through curriculum-style learning, an avenue we plan to pursue in future work.
PBEBench-Lite is already challenging for many models, especially non-reasoning ones, indicating that inductive reasoning requires long chains of thought at test time. Experiments with the strongest open and closed-source models on PBEBench show that while they handle moderate complexity, performance steadily declines as complexity, mainly driven by ground-truth cascade length, increases. Even with intensive scaling strategies like larger sampling and token budgets, performance eventually saturates, highlighting the reasoning limits of current state-of-the-art models. Nonetheless, results are promising and surpass prior work \citep{naik2024can, naik2025programming}, pointing to a bright future for solving forward reconstruction problems with LLMs. Moreover, our automated, scalable data generation with controllable complexity could enable increasingly complex synthetic training data, potentially enhancing PBE and inductive reasoning in open-weight models via curriculum-style learning, an avenue we plan to pursue in future work.
% Firstly, PBEBench-Lite is already challenging for many models, especially non-reasoning ones, suggesting that inductive reasoning requires long chains of thought at test time. Experiments with the strongest open and closed-source models on the more realistic PBEBench dataset show that while these models solve problems up to a certain complexity, performance declines steadily as complexity, largely driven by ground-truth cascade length, increases. Even with computationally intensive scaling strategies such as larger sampling and token budgets, performance eventually saturates, revealing reasoning barriers and the limits of current state-of-the-art models. Nonetheless, these results are promising and already surpass prior work \citep{naik2024can, naik2025programming}, indicating a bright future for solving forward reconstruction problems with LLMs. Finally, the automated, scalable generation of data with controllable complexity enabled by our pipeline opens the door to increasingly complex synthetic training data, which could enhance PBE and inductive reasoning abilities of open-weight models through curriculum-style learning, an avenue we plan to pursue in future work.



% Local Variables:
% TeX-master: "../iclr2026_conference"
% TeX-engine: xetex
% mode: LaTeX
% End:

